Fortuna: A Library for Uncertainty Quantification in Deep Learning

We present Fortuna, an open-source library for uncertainty quantification in deep learning. Fortuna supports a range of calibration techniques, such as conformal prediction that can be applied to any trained neural network to generate reliable uncertainty estimates, and scalable Bayesian inference methods that can be applied to Flax-based deep neural networks trained from scratch for improved uncertainty quantification and accuracy. By providing a coherent framework for advanced uncertainty quantification methods, Fortuna simplifies the process of benchmarking and helps practitioners build robust AI systems.

==> Fortuna MLOSS/coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Fortuna: A Library for Uncertainty Quantification in Deep Learning}'' to the \emph{Journal of Machine Learning Research (Open-Source Software)}.

Our manuscript introduces Fortuna, an open-source library for uncertainty quantification in deep learning. The library is actively maintained within AWS. It accounts for one full-time core developers, and several part-time in-house developers. Contributions from the community are also growing. The library was released in December 2022, and at the time of writing it counts 417 stars and 29 forks.

We suggest the following action editors for our submission.

Action Editors:
\begin{itemize}
    \item \red{Silvia Chiappa, DeepMind (chiappa.silvia@gmail.com)}
    \item \red{Stephan Mandt, University of Columbia (mandt@uci.edu)}
    \item \red{Samy Bengio, Apple (bengio@apple.com)}
\end{itemize}

We do not have specific referee suggestions.

Our submission has the following keywords: \red{uncertainty-quantification}, \red{conformal-prediction}, \red{bayesian-inference}, \red{calibration}, \red{deep-learning}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Gianluca Detommaso, AWS}\\
\red{Alberto Gasparin, Amazon}\\
\red{Michele Donini, AWS}\\
\red{Matthias Seeger, AWS}\\
\red{Andrew Gordon Wilson, AWS \& New York University}\\
\red{Cedric Archambeau, AWS}

\end{document}








































==> coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Fortuna: A Library for Uncertainty Quantification in Deep Learning}'' to the \emph{Journal of Machine Learning Research (Open-Source Software)}.

Our manuscript introduces Fortuna, an open-source library for uncertainty quantification in deep learning. The library is actively maintained within AWS. It accounts for one full-time core developers, and several part-time in-house developers. Contributions from the community are also growing. The library was released in December 2022, and at the time of writing it counts 417 stars and 29 forks.

We suggest the following action editors for our submission.

Action Editors:
\begin{itemize}
    \item \red{Silvia Chiappa, DeepMind (chiappa.silvia@gmail.com)}
    \item \red{Stephan Mandt, University of Columbia (mandt@uci.edu)}
    \item \red{Samy Bengio, Apple (bengio@apple.com)}
\end{itemize}

We do not have specific referee suggestions.

Our submission has the following keywords: \red{uncertainty-quantification}, \red{conformal-prediction}, \red{bayesian-inference}, \red{calibration}, \red{deep-learning}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Gianluca Detommaso, AWS}\\
\red{Alberto Gasparin, Amazon}\\
\red{Michele Donini, AWS}\\
\red{Matthias Seeger, AWS}\\
\red{Andrew Gordon Wilson, AWS \& New York University}\\
\red{Cedric Archambeau, AWS}

\end{document}







































